MAS-Attention: Memory-Aware Stream Processing for Attention Acceleration on Resource-Constrained Edge Devices

The advent of foundation models have revolutionized various fields, enabling unprecedented task accuracy and flexibility in computational linguistics, computer vision and other domains. Attention mechanism has become an essential component of foundation models, due to their superb capability of capturing correlations in a sequence. However, attention results in quadratic complexity in memory and compute as the context length grows. Although many fusion-based exact attention acceleration algorithms have been developed for datacenter-grade GPUs and accelerators leveraging multi-core parallelism and data locality, yet it remains a significant challenge to accelerate attention on resource-constrained edge neural accelerators with limited compute units and stringent on-chip caches. In this paper, we propose a scheme for exact attention inference acceleration on memory-constrained edge accelerators, by parallelizing the utilization of heterogeneous compute units, i.e., vector processing units and matrix processing units. Our method involves scheduling workloads onto these different compute units in a multi-tiered tiling scheme to process tiled vector workloads and matrix workloads in attention as two streams, respecting the workload dependencies. We search for tiling factors to maximize the parallelization of both compute units while considering I/O overhead, and propose a proactive cache overwrite strategy to avoid undesirable cache spills in reality. Extensive results based on open-sourced simulation frameworks show up to 2.75x speedup and 54% reduction in energy consumption as compared to the state-of-the-art attention fusion method (FLAT) in the edge computing scenario. Further experiments on a real-world edge neural processing unit demonstrate speedup of up to 1.76x for attention as compared to FLAT, without affecting model output accuracy.

==> sections/experiment.tex <==
\label{sec:experiment}
    
    
\subsection{Experimental Setup}

    
Our experiments were conducted on a system equipped with an Intel(R) Xeon(R) Gold 6140 CPU @ 2.30GHz, utilizing a single thread in execution. For simulating our experiment, we utilized the TileFlow framework \cite{zheng2023tileflow}. The custom edge hardware architecture designed for this study in TileFLow features 16nm technology, two cores, each with two sub-cores, and a hierarchical memory system as outlined in \autoref{table:hardware}. The designed DRAM has a bandwidth of 30GB/sec and a total size of 6GB. The L1 cache is designed as a stack of four units, each with a total size of 1256KB. The 16x16 Processing Elements (PEs) for MAC and vector unit have access to a separate L0 register file, organized in a 256 mesh. The architecture operates at a frequency of 3.75GHz. Additionally, we evaluated our algorithm on real hardware, specifically using an edge device with DaVinci DNN Accelerator, to validate its practical applicability and performance.\\
\begin{table}[h]
\centering
\caption{Edge Hardware Specification}
\label{table:hardware}
\renewcommand{\arraystretch}{1.3}
\scriptsize
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\textbf{Cores} & \textbf{Sub-Cores} & \textbf{\# of PEs} & \textbf{L1 Size} & \textbf{DRAM Size} & \textbf{DRAM BW} \\ \hline
2 & 2 & 16×16  & 5024KB & 6GB & 30GB/sec \\ \hline
\end{tabular}
\end{table}
The workload for our experiments centers on the inference of attention layers in transformer-based networks. We considered a diverse set of networks with varying dimensions in their attention layers to ensure a comprehensive evaluation.
We evaluated three distinct algorithms: Naive Layer-Wise execution of the attention layer, FLAT, and our proposed algorithm, MAS-Attention. The performance metrics used in this study include execution time analysis, power efficiency evaluation, off-chip memory footprint analysis, component-wise energy breakdown, and memory hierarchy utilization. Our results show that MAS-Attention consistently outperforms the other two algorithms across all evaluated metrics, demonstrating superior efficiency and performance.

\begin{table}[h]
\centering
\caption{Network Configuration and Hyper-parameters}
\label{table:modelspecs}
\renewcommand{\arraystretch}{1.4}
\scriptsize
\begin{tabular}{|c|c|c|c|c|}
\hline
\textbf{Network Name} & \textbf{\#Heads} & \textbf{\#Seq} & \textbf{Hidden size} & \textbf{Emb\textsubscript{K,V}} \\ \hline
BERT-Base \& T5-Base & 12 & 512 & 768 & 64 \\ \hline
BERT-Large \& T5-Large & 16 & 512 & 1024 & 64 \\ \hline
BERT-Small & 8 & 512 & 512 & 64 \\ \hline
Llama3-8B \& T5-3B (T5-XL) & 32 & 512 & 4096 & 128 \\ \hline
T5-Mini \& T5-Small & 8 & 512 & 256 & 32 \\ \hline
ViT-B/14 & 12 & 196 & 768 & 64 \\ \hline
ViT-L/14 & 16 & 196 & 1024 & 64 \\ \hline
ViT-H/14 & 16 & 196 & 1280 & 80 \\ \hline
ViT-B/16 & 12 & 256 & 768 & 64 \\ \hline
ViT-L/16 & 16 & 256 & 1024 & 64 \\ \hline
ViT-H/16 & 16 & 256 & 1280 & 80 \\ \hline
XLM & 8 & 512 & 1024 & 128 \\ \hline
\end{tabular}
\end{table}


\subsection{Execution Time Analysis}

The execution time analysis is a critical aspect of evaluating the performance of algorithms, as it directly determines the cycles, throughput, and responsiveness of a system. Due to its importance, this analysis was included as a key part of the experiments in this paper. \autoref{fig:cycleAnalysis} quantitatively compares the normalized cycle counts of three algorithms—Naive Layer-Wise, FLAT, and MAS-Attention—in tileflow framework across all networks as outlined in \autoref{table:modelspecs}. Our findings indicate that MAS-Attention algorithm yields a significant performance enhancement, with a speedup of 2x relative to FLAT and 4.63x relative to Layer-Wise, in the case of BERT-Base and T5-Base networks. Similarly, for BERT-Large and T5-Large networks, MAS-Attention exhibits a speedup of 1.75x compared to FLAT and 5.26x compared to Layer-Wise. Furthermore, in the case of the Llama3-8B and T5-3B network, MAS-Attention demonstrates a speedup of 1.12x relative to FLAT and 3.06x relative to Layer-Wise. Consistent performance improvements are observed across all tested networks. In addition to the TileFlow framework experiments, further experiments were conducted using an edge device with DaVinci DNN accelerator. Results, detailed in \autoref{fig:CPRO_cycleAnalysis}, show that MAS-Attention continues to outperform other methods. For instance, in the BERT-Base \& T5-Base network, MAS-Attention achieves a speedup of 1.37x over FLAT and 2.18x over Layer-Wise. Similar trends are seen across other networks, such as BERT-Large \& T5-Large and Llama3-8B \& T5-3B (T5-XL), where MAS-Attention consistently provides notable speedups. In the case of the Vision Transformer (ViT) networks, MAS-Attention exhibits significant improvements, with speedups of up to 1.76x over FLAT and 3.50x over Layer-Wise. The results underscore the advanced optimization capabilities of MAS-Attention, making it a preferable choice for optimizing execution time in high-performance computing applications. Detailed speedup values for all networks are included in \autoref{table:cycle_counts_and_speedup} and \autoref{table:normalized_cycle_counts_and_speedup_CPRO} in the supplementary material.

% % one columns wide
% \begin{figure}[ht]
%   \centering
%   \includegraphics[width=\columnwidth]{figs/cycleAnalysis.png}
%   \caption{Normalized Cycle Comparison Across Networks for Different Methods on Simulated Edge Hardware}
%   \label{fig:cycleAnalysis}
% \end{figure}

\begin{figure}[ht]
  \centering
  \includegraphics[width=\columnwidth]{figs/CPRO_cycleAnalysis_normalized.png}
  \caption{Normalized Cycle Comparison Across Networks for Different Methods on Edge device with DaVinci DNN Accelerator}
  \label{fig:CPRO_cycleAnalysis}
\end{figure}


\begin{table*}[ht]
    \centering
    \caption{Cycles and Speedup Comparisons}
    \label{tab:cycles_speedup}
    \small
    \resizebox{\textwidth}{!}{
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
        \hline
        \multirow{2}{*}{\textbf{Network Name}} & \multicolumn{5}{c|}{\textbf{Cycles }($10^6$)} & \multicolumn{4}{c|}{\textbf{Speedup (MAS-Attention vs. Others)}} \\ \cline{2-10}
         & Layer-Wise & Soft-Pipe & FLAT & TileFlow & MAS-Attention & Layer-Wise & Soft-Pipe & FLAT & TileFlow \\ \hline
        BERT-Base \& T5-Base & 3.637 & 2.064 & 1.573 & 0.799 & 0.786 & 4.625 & 2.625 & 2.000 & 1.016 \\ \hline
        BERT-Large \& T5-Large & 5.505 & 2.753 & 1.835 & 1.311 & 1.049 & 5.250 & 2.625 & 1.750 & 1.250 \\ \hline
        BERT-Small & 2.753 & 1.376 & 0.918 & 0.655 & 0.524 & 5.250 & 2.625 & 1.750 & 1.250 \\ \hline
        Llama3-8B \& T5-3B (T5-XL) & 12.845 & 8.389 & 4.719 & 5.243 & 4.194 & 3.063 & 2.000 & 1.125 & 1.250 \\ \hline
        T5-Mini \& T5-Small & 2.228 & 1.180 & 0.721 & 0.328 & 0.262 & 8.500 & 4.500 & 2.750 & 1.250 \\ \hline
        ViT-B/14 & 0.612 & 0.381 & 0.266 & 0.263 & 0.151 & 4.063 & 2.531 & 1.766 & 1.750 \\ \hline
        ViT-L/14 & 1.242 & 0.508 & 0.354 & 0.351 & 0.201 & 6.188 & 2.531 & 1.766 & 1.750 \\ \hline
        ViT-H/14 & 1.355 & 0.558 & 0.405 & 0.439 & 0.251 & 5.400 & 2.225 & 1.613 & 1.750 \\ \hline
        ViT-B/16 & 1.081 & 0.590 & 0.426 & 0.249 & 0.197 & 5.500 & 3.000 & 2.167 & 1.266 \\ \hline
        ViT-L/16 & 1.311 & 0.786 & 0.524 & 0.332 & 0.262 & 5.000 & 3.000 & 2.000 & 1.266 \\ \hline
        ViT-H/16 & 1.376 & 0.852 & 0.590 & 0.414 & 0.328 & 4.200 & 2.600 & 1.800 & 1.263 \\ \hline
        XLM & 4.194 & 2.097 & 1.180 & 1.311 & 1.049 & 4.000 & 2.000 & 1.125 & 1.250 \\ \hline
    \end{tabular}
    }
\end{table*}

\subsection{Power Efficiency Evaluation}
Optimizing power efficiency is essential when deploying large transformer-based models, particularly on resource-constrained devices, as it significantly influences power consumption, battery life, and thermal management, ultimately affecting the overall performance and reliability of the device. As shown in \autoref{fig:energyAnalysis}, our evaluation of power efficiency, measured as cumulative energy consumption across all levels of memory hierarchy and processing elements in the hardware, demonstrates the effectiveness of our proposed MAS-Attention algorithm. Across all tested networks, MAS-Attention consistently matches or outperforms FLAT method, and outperforms the Naive Layer-Wise approach. For example, on the BERT-Large and T5-Large networks, MAS-Attention achieves 1.25x power efficient compared to FLAT and 1.66x more efficient than Naive Layer-Wise method. Similar improvements are observed across other models, such as ViT-B14, where MAS-Attention achieves a power efficiency of 1.47x compared to FLAT and 1.95x compared to Layer-Wise method. These results highlight the significant advantage of MAS-Attention in minimizing power consumption during inference, making it a compelling choice for applications requiring both performance and energy efficiency. Detailed normalized energy consumption values for all networks are included in \autoref{table:energy_consumption_and_reduction_factors} in the supplementary material.

% \begin{figure}[ht]
%   \centering
%   \includegraphics[width=\columnwidth]{figs/energyAnalysis.png}
%   \caption{Normalized Power Consumption Comparison Across Networks for Different Methods}
%   \label{fig:energyAnalysis}
% \end{figure}

\begin{table*}[ht]
    \centering
    \caption{Energy Consumption and Savings Comparisons}
    \label{tab:energy_savings}
    \small
    \resizebox{\textwidth}{!}{
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
        \hline
        \multirow{2}{*}{\textbf{Network Name}} & \multicolumn{5}{c|}{\textbf{Energy Consumption ($10^9$ nJ)}} & \multicolumn{4}{c|}{\textbf{Energy Savings (MAS-Attention vs. Others)}} \\ \cline{2-10}
         & Layer-Wise & Soft-Pipe & FLAT & TileFlow & MAS-Attention & Layer-Wise & Soft-Pipe & FLAT & TileFlow \\ \hline
        BERT-base \& T5-Base & 37.2084 & 49.6067 & 12.6559 & 27.5977 & 12.4053 & 66.67\% & 75.00\% & 1.98\% & 55.05\% \\ \hline
        BERT-large \& T5-Large & 28.1047 & 65.6715 & 21.1115 & 38.0645 & 16.9436 & 39.69\% & 74.20\% & 19.75\% & 55.49\% \\ \hline
        BERT-small & 20.2181 & 24.3363 & 10.5558 & 19.0323 & 8.3585 & 58.65\% & 65.64\% & 20.80\% & 56.08\% \\ \hline
        Llama3-8B \& T5-3B (T5-XL) & 179.3090 & 186.4630 & 63.2517 & 147.5020 & 63.2413 & 64.73\% & 66.08\% & 0.02\% & 57.12\% \\ \hline
        T5-Mini \& T5-Small & 12.4343 & 11.2692 & 8.7439 & 7.5122 & 4.7458 & 61.83\% & 57.90\% & 45.71\% & 36.83\% \\ \hline
        ViT-B/14 & 3.7201 & 7.3764 & 2.8029 & 4.1359 & 1.9027 & 48.87\% & 74.21\% & 32.11\% & 54.00\% \\ \hline
        ViT-L/14 & 5.5388 & 7.3351 & 5.6481 & 7.4280 & 2.5961 & 53.13\% & 64.61\% & 54.03\% & 65.05\% \\ \hline
        ViT-H/14 & 6.5851 & 9.1203 & 4.7409 & 6.7832 & 3.1621 & 51.98\% & 65.34\% & 33.27\% & 53.38\% \\ \hline
        ViT-B/16 & 5.3226 & 5.8284 & 3.3504 & 7.1188 & 3.2391 & 39.16\% & 44.42\% & 3.34\% & 54.49\% \\ \hline
        ViT-L/16 & 9.4031 & 6.9843 & 6.3164 & 9.4018 & 4.2180 & 55.14\% & 39.61\% & 33.21\% & 55.14\% \\ \hline
        ViT-H/16 & 11.1599 & 15.4138 & 6.8026 & 11.4753 & 5.1560 & 53.81\% & 66.55\% & 24.22\% & 55.09\% \\ \hline
        XLM-Base & 35.7857 & 46.4846 & 15.8130 & 36.8755 & 15.5840 & 56.45\% & 66.47\% & 1.45\% & 57.74\% \\ \hline
    \end{tabular}
    }
\end{table*}

\subsection{Component-Wise Energy Breakdown}
Component-wise energy breakdown is crucial as it reveals the energy efficiency of each component, identifies bottlenecks, and enables targeted optimization. This approach facilitates improved energy consumption, thermal management, and performance across different system layers, enhancing overall system efficiency and sustainability. In this analysis, we will focus on Off-Chip (DDR), On-Chip (L1, L0), and PEs energy consumption.
\subsubsection{Off-Chip Memory}
Compared to Layer-Wise calculation, FLAT and MAS-Attention significantly reduce off-chip energy consumption. This reduction is achieved by minimizing the number of necessary accesses to DRAM, eliminating the need to store intermediate Logit and Attend matrices off-chip. Notably, the off-chip energy consumption for MAS-Attention is consistently same as or greater than that of FLAT. This phenomenon arises when MAS-Attention requires reloading specific chunks of data components, specifically $K$ and $V$ matrices, which were overwritten during the pipelining stages on chip. This reloading process necessitates additional energy consumption, as these data components must be accessed again from DRAM, thereby increasing the overall energy expenditure.
\subsubsection{On-Chip Memory}
Layer-Wise method generally exhibit higher L1 energy consumption compared to FLAT and MAS-Attention methods, indicating less efficient memory utilization. This trend is evident across multiple networks, with Layer-Wise generally consuming the most energy, followed by FLAT and MAS-Attention. Similarly, L0 energy consumption shows that Layer-Wise methods tend to be less efficient. These observations suggest that FLAT and MAS-Attention methods achieve superior energy efficiency in on-chip memory utilization, which is crucial for optimizing overall system performance.

\subsubsection{PEs}
The energy consumption in PEs remains constant across different algorithms for each network. This consistency arises because the actual computation required by different algorithms is the same, with differences only in the scheduling process, which impacts the energy consumption of other hardware components.

This comprehensive component-wise analysis, corroborated by the data presented in \autoref{fig:energyConsumptionBreakdown_v2} and meticulously detailed in \autoref{table:energy_consumption_Breakdown}, underscores the efficiency of our method across all system layers for the tested networks.
% \begin{figure}[ht]
%   \centering
%   \includegraphics[width=\columnwidth]{energyConsumptionBreakdown.png}
%   \caption{Energy Consumption Breakdown}
%   \label{fig:energyConsumptionBreakdown}
% \end{figure}

\begin{figure}[ht]
  \centering
  \includegraphics[width=\columnwidth]{figs/energyConsumptionBreakdown_v2.png}
  \caption{Energy Consumption Breakdown}
  \label{fig:energyConsumptionBreakdown_v2}
\end{figure}

\subsection{Off-Chip Memory Footprint Analysis}

Optimizing off-chip memory footprint is crucial for ensuring efficient resource allocation, scalability, and reliability in large-scale transformer-based models. Excessive off-chip memory access can lead to significant performance bottlenecks, increased latency, and a heightened risk of data errors and system crashes. In this context, a comprehensive off-chip memory footprint analysis is essential for identifying opportunities for optimization and mitigating potential issues. As shown in \autoref{table:Off_Chip_Memory_Savings} our proposed MAS-Attention algorithm demonstrates superior performance in this regard, achieving an average off-chip memory saving of 73.41\% to 99.97\% across various sequence lengths and models, compared to the naive method.
\begin{table}[h]
\centering
\caption{Comparison of Off-Chip memory Requirements for Attention Layer with 8K sequence size in Llama3-8B}
\label{table:Llama3_8B_Parameters_OffChip_Memory_Req}
\scriptsize % Reduce font size
\setlength{\tabcolsep}{3pt} % Reduce space between columns
\renewcommand{\arraystretch}{1.2} % Adjust row height
\begin{tabular}{|C|c|c|c|c|c|}
\hline
\textbf{Variables} & \textbf{Data Shape} & \textbf{Data Size (MB)} & \multicolumn{3}{c|}{\textbf{Off-Chip Memory Requirement}} \\ \cline{4-6} 
 &  &  & \textbf{Layer-Wise} & \textbf{FLAT} & \textbf{MAS-Attention} \\ \hline
\begin{math}Q\end{math} & (1, 32, 8K, 128) & 65.536 & \cmark & \cmark & \cmark \\ \hline
\begin{math}K\end{math} & (1, 32, 8K, 128) & 65.536 & \cmark & \cmark & \cmark \\ \hline
\begin{math}V\end{math} & (1, 32, 8K, 128) & 65.536 & \cmark & \cmark & \cmark \\ \hline
\begin{math}C\end{math} & (1, 32, 8K, 8K) & 4096 & \cmark & \xmark & \xmark \\ \hline
\begin{math}P\end{math} & (1, 32, 8K, 8K) & 4096 & \cmark & \xmark & \xmark \\ \hline
\begin{math}O\end{math} & (1, 32, 8K, 128) & 65.536 & \cmark & \cmark & \cmark \\ \hline
\end{tabular}
\end{table}
In our analysis, MAS-Attention and FLAT algorithms both exhibit similar, yet impressive performance in optimizing off-chip memory requirements. By focusing on the Llama3-8B model with an 8K sequence length, as shown in \autoref{table:Llama3_8B_Parameters_OffChip_Memory_Req}, we demonstrate the substantial memory savings achieved by these methods. 
\begin{table*}[ht]
\caption{Off-Chip Memory Saving of MAS-Attention vs. Layer-Wise}
\label{table:Off_Chip_Memory_Savings}
\centering
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\textbf{Seq. Length} & \textbf{512} & \textbf{2K} & \textbf{4K} & \textbf{8K} & \textbf{16K} & \textbf{32K} & \textbf{64K} & \textbf{128K} & \textbf{256K} & \textbf{512K} \\ \hline
BERT-Base/T5-Base & 80\% & 93.98\% & 96.9\% & 98.43\% & 99.21\% & 99.6\% & 99.8\% & 99.9\% & 99.95\% & 99.98\% \\ \hline
BERT-Large/T5-Large & 80\% & 93.98\% & 96.9\% & 98.43\% & 99.21\% & 99.6\% & 99.8\% & 99.9\% & 99.95\% & 99.98\% \\ \hline
Llama3-8B/T5-3B & 66.67\% & 88.65\% & 93.98\% & 96.9\% & 98.43\% & 99.21\% & 99.6\% & 99.8\% & 99.9\% & 99.95\% \\ \hline
XLM & 66.67\% & 88.65\% & 93.98\% & 96.9\% & 98.43\% & 99.21\% & 99.6\% & 99.8\% & 99.9\% & 99.95\% \\ \hline
\textbf{Average} & \textbf{73.41\%} & \textbf{91.81\%} & \textbf{95.69\%} & \textbf{97.66\%} & \textbf{98.96\%} & \textbf{99.4\%} & \textbf{99.7\%} & \textbf{99.85\%} & \textbf{99.925\%} & \textbf{99.9675\%} \\ \hline
\end{tabular}
\end{table*}
The off-chip memory footprints for $Q, K,$ and $V$ matrices, each with a size of (1, 32, 8K, 128), are 65.536MB respectively. Additionally, $C$ and $P$ matrices, both sized at (1, 32, 8K, 8K), consume 4096MB each. The output matrix $O$, also sized at (1, 32, 8K, 128), requires another 65.536MB. In total, the naive layer-wise method incurs a significant off-chip memory footprint of 8454.144MB. Conversely, MAS-Attention and FLAT algorithms, by eliminating the need for storing $C$ and $P$ matrices off-chip, reduce the memory footprint dramatically to just 262.144MB. This represents a remarkable 97\% reduction in off-chip memory requirements.

\begin{table*}[ht]
\caption{Data Access Between Different Memory Hierarchies of MAS-Attention over FLAT}
\label{table:Memory_Hierarchy_Utilization}
\centering
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{\textbf{Network}} & \multirow{2}{*}{\textbf{Speedup}} & \multirow{2}{*}{\textbf{Energy consumption}} & \multicolumn{2}{c|}{\textbf{DRAM}} & \multicolumn{2}{c|}{\textbf{L1}} & \multicolumn{2}{c|}{\textbf{L0}} \\ \cline{4-9}
 &  &  & \textbf{Write} & \textbf{Read} & \textbf{Write} & \textbf{Read} & \textbf{Write} & \textbf{Read} \\ \hline
BERT-Base \& T5-Base & 2.000000 & 0.980199 & 1.0 & 1.500006 & 1.369566 & 1.914634 & 2.166263 & 2.296295 \\ \hline
BERT-Large \& T5-Large & 1.750000 & 0.802577 & 1.0 & 1.500002 & 3.192317 & 2.877193 & 3.262662 & 2.533333 \\ \hline
BERT-Small & 1.750000 & 0.791842 & 1.0 & 1.000000 & 3.153838 & 2.877193 & 3.262679 & 2.533335 \\ \hline
Llama3-8B \& T5-3B & 1.125000 & 0.999836 & 1.0 & 1.499998 & 3.277780 & 3.999993 & 4.464783 & 4.333341 \\ \hline
T5-Mini \& T5-Small & 2.750000 & 0.542757 & 1.0 & 1.000000 & 0.844156 & 2.421048 & 3.057102 & 2.476182 \\ \hline
ViT-B/14 & 1.765625 & 0.678845 & 1.0 & 1.000000 & 0.426859 & 1.433161 & 2.017933 & 2.013889 \\ \hline
ViT-B/16 & 2.166667 & 0.966783 & 1.0 & 1.000000 & 2.099996 & 2.928582 & 2.451059 & 1.900004 \\ \hline
ViT-H/14 & 1.612500 & 0.666975 & 1.0 & 1.000000 & 0.946071 & 2.834326 & 3.830479 & 3.450988 \\ \hline
ViT-H/16 & 1.800000 & 0.757944 & 1.0 & 1.000000 & 1.000000 & 3.063491 & 3.203709 & 2.349209 \\ \hline
ViT-L/14 & 1.765625 & 0.459632 & 1.0 & 1.000000 & 0.597176 & 1.898863 & 3.843158 & 3.619043 \\ \hline
ViT-L/16 & 2.000000 & 0.667775 & 1.0 & 1.000000 & 2.666664 & 2.180556 & 2.621366 & 1.722223 \\ \hline
XLM & 1.125000 & 0.985518 & 1.0 & 1.000000 & 3.222218 & 4.000000 & 3.235135 & 2.583330 \\ \hline
\end{tabular}
\end{table*}

\subsection{Memory Hierarchy Utilization}
Memory access patterns significantly influence both speed and energy consumption, particularly in memory-intensive computations such as attention mechanism. By examining how MAS-Attention algorithm interacts with all levels of the memory hierarchy, we can elucidate the factors contributing to its superior performance over FLAT algorithm. This analysis not only optimizes memory usage but also reduces overall latency and enhances all-inclusive system efficiency.
From \autoref{table:Memory_Hierarchy_Utilization}, several critical differences between MAS-Attention and FLAT algorithms memory utilization can be discerned:

\subsubsection{Consistent Write Operations to DRAM}
Both MAS-Attention and FLAT algorithms exhibit an identical number of write operations to DRAM. This uniformity arises because both algorithms confine their DRAM write operations to the final result of the attention block (\begin{math}O\end{math}), eschewing the need to write intermediate results to DRAM. Instead, these intermediate results are processed entirely on-chip, thereby minimizing off-chip memory accesses and enhancing overall efficiency.

\subsubsection{Selective Increase in DRAM Read Operations in MAS-Attention}
MAS-Attention matches or exceeds the DRAM read operations of FLAT for certain networks. Notably, for BERT-Base \& T5-Base (1.500006), BERT-Large \& T5-Large (1.500002), and Llama3-8B \& T5-3B (1.499998), MAS-Attention shows increased DRAM read operations. This phenomenon arises because MAS-Attention requires reloading specific data chunks, particularly $K$ and $V$ matrices, which may have been overwritten during the pipelining stages in SRAM. This reloading from DRAM is limited to \begin{math}K\end{math} and \begin{math}V\end{math} matrices because the first operand of both matrix multiplications, \begin{math}Q\end{math} from first and \begin{math}P\end{math} from second matrix multiplication, remains untouched. Maintaining the integrity of \begin{math}P\end{math} is critical because \begin{math}Softmax(QK^T)\end{math} operation occurs on-chip, and any overwriting would preclude reloading from alternative memory sources. Our findings indicate that preserving first operands of matrix multiplications including \begin{math}Q\end{math} on-chip without overwriting insures the final results of the operation's correctness.

\subsubsection{Increased On-Chip Read/Write Operations}
MAS-Attention algorithm necessitates a higher frequency of on-chip read/write operations compared to FLAT due to its pipelined processing scheme. This pipelining requires more frequent data accesses within the on-chip memory, contrasting with the sequential processing approach of the FLAT algorithm. Although this increased on-chip data movement demands more read/write operations, it enables MAS-Attention to maintain higher throughput and better exploit the memory hierarchy, resulting in improved performance metrics.

These insights underscore the significance of memory hierarchy utilization in designing efficient algorithms. By leveraging on-chip processing and strategically managing memory accesses, MAS-Attention achieves notable speedup and energy efficiency over FLAT, despite the increased on-chip read/write operations. This analysis paves the way for further optimizations in memory-bound computation tasks, facilitating the development of more efficient and powerful algorithmic implementations.

==> sections/future_work.tex <==
\label{sec:future_work}
Future work will focus on extending MAS-Attention to support training, as the current implementation is designed specifically for inference. Training introduces additional computational complexity, particularly in backpropagation, and optimizing MAS-Attention to efficiently manage these tasks on resource-constrained edge devices presents a compelling challenge. 

Another key direction is adapting MAS-Attention for cloud-based environments. While this work targets edge devices, leveraging MAS-Attention's memory-efficient, pipelined execution within the cloud could offer significant benefits, particularly for large-scale distributed training and inference, thereby extending its applicability across both edge and cloud systems.

% TODO: combine this with conclusion; shorter future work (no need to mention for cloud, for training, how to do on-device training); first conclusion, then future work

==> sections/related_work.tex <==
\label{sec:relatedwork}
    % Overall structure:
    %     1. Acceleration methods for transformer large model. 1) Approximate acceleration methods; 2) Exact acceleration methods
    %     2. AI compiler, e.g., Halide, TVM, oneDNN. Introduce auto-scheduler for operators. Graph level optimization, e.g., graph stitch. Pipelining is not considered


   % Acceleration methods for transformer-based foundation models can be categorized into three main directions: approximate acceleration, parallelization-based exact acceleration, and fusion-based exact acceleration. In this section, we introduce related works within these three research areas. 

    \textbf{Approximate Acceleration Algorithms:}
    For approximate acceleration methods of transformer-based foundation models, a key research focus has been on compressing the model size while maintaining comparable performance. 
    Techniques such as palletization \cite{cho2021dkm, tabani2021improving, wang2020cluster, appleCoreML}, quantization \cite{liu2021post, lin2021fq, wang2022deep, li2022q, piao2022sensimix, yao2022zeroquant, li2023vit, yu2023boost}, and pruning \cite{mao2021tprune, peng2021accelerating, yu2022unified, yu2022width} have been extensively studied for clustering, quantizing, or pruning weight parameters at various levels of granularity. 
    These approaches result in smaller model sizes with similar performance, thereby alleviating memory challenges during deployment and accelerating inference time. 
    Knowledge distillation techniques \cite{sun2019patient, wang2020minilm, wang2020minilmv2, ganesh2021compressing, huang2024knowledge, gupta2024progressive}, which involve transferring the knowledge from a large pre-trained teacher model to a smaller student model, are also widely studied. These methods effectively reduce the model size and/or the number of inference steps, thereby accelerating the inference process for foundation models. 
    
    Besides applying acceleration techniques to model weights, compression techniques for the attention layers in transformer-based foundation models are also extensively researched. 
    Leveraging the sparsity of the attention blocks, methods such as token merging \cite{bolya2022token, bolya2023token, kim2024token, smith2024todo}, KV cache quantization and compression \cite{pope2023efficiently, hooper2024kvquant, zhang2024h2o, ge2023model, li2024snapkv} have been widely studied to accelerate the inference time of large vision and language models. 
    While these approximate acceleration algorithms can negatively impact model performance, they are orthogonal to our proposed MAS-Attention. When combined, they can further reduce model inference time during deployment. 

    \textbf{Exact Acceleration Algorithms:}
    Parallelization-based acceleration algorithms are another prominent research area for speeding up exact attention computation. 
    FlashAttention \cite{dao2022flashattention} and its related works \cite{dao2023flashattention, dao2023flashdecoding, hong2023flashdecoding++, nayak2024fusemax} leverage the multi-core capabilities of GPUs to accelerate the attention mechanism through parallelization. 
    By using fusion dataflows and parallelizing the computation of attention slices, FlashAttention enhances GPU utilization and reduces the inference runtime of the attention mechanism. 

    Beyond accelerating just the attention blocks, several works propose parallelization and computational resource allocation algorithms to accelerate the end-to-end inference of foundation models. 
    Examples include Microsoft's Spitwise \cite{patel2023splitwise}, Ring Attention \cite{liu2023ring}, and Apple's KV-Runahead \cite{cho2024kv}, which allocate computational resources within and across multiple GPUs based on the computational complexity of the prompt and decoding phases of LLM inference, utilizing parallelization algorithms to speed up overall inference time.

    These parallelization-based acceleration algorithms are widely deployed in cloud-based LLM inference services, which have multiple hardware accelerators like GPUs, each with numerous computational cores for parallel processing. 
    However, on edge devices, harnessing the power of parallel computing requires a carefully designed attention dataflow, which is central to our proposed MAS-Attention. 

    \textbf{Fusion-based Exact Acceleration Algorithms:}
    Before transformer-based foundation models became widely adopted, the dataflows for individual operators, such as convolution \cite{chen2016eyeriss, dave2019dmazerunner, du2015shidiannao, gao2017tetris, gao2019tangram, kao2020gamma, lu2017flexflow, parashar2019timeloop, yang2020interstellar, yazdanbakhsh2018ganax, zhang2015optimizing, wei2017automated} and matrix multiplication \cite{venkataramani2017scaledeep, song2019hypar, shao2019simba, jouppi2017datacenter, kumar2021data}, were designed to accelerate the runtime of these operators on DNN accelerators through the Layer-Wise execution. 
    In addition to the dataflow designed for individual operators, fusion-based acceleration algorithms have been proposed to enhance the runtime of either computational sub-graph patterns or entire neural networks end-to-end. 
    
    Fusion-based algorithms have been developed for commonly used computational patterns, such as MLP layers \cite{ivanov2021data, niu2021dnnfusion} that include matrix multiplication and activation operators, as well as multiple convolution operators \cite{alwani2016fused, wei2018tgpa}. 
    To optimize entire neural networks end-to-end, graph fusion-based methods have been widely adopted in tensor compilers \cite{gao1993collective, kjolstad2017tensor, chen2018learning, baghdadi2019tiramisu, googleXLA} and neural network acceleration libraries \cite{appleCoreML, appleAccelerateF, appleMetalPSG, NvidiaTensorRT, zhou2022exploring, aminabadi2022deepspeed}. 
    These methods fuse multiple operators into a single kernel, allowing intermediate data to be computed and stored in on-chip memory. This reduces the overhead of reading and writing intermediate data between off-chip and on-chip memory, as well as the kernel launch time. 

    Furthermore, with the widespread adoption of transformer-based foundation models, there has been significant interest in developing efficient fusion dataflows for attention layers. 
    FlashAttention \cite{dao2022flashattention, dao2023flashattention, dao2023flashdecoding, hong2023flashdecoding++}, FuseMax \cite{nayak2024fusemax}, and oneDNN \cite{li2024onednn} have proposed fusion dataflows to accelerate the attention mechanism with parallelization in cloud scenarios. 
    In contrast, FLAT \cite{kao2023flat} leverages on-chip memory to propose a fusion dataflow for attention mechanisms on edge devices, reducing the overhead of reading and writing large intermediate data between off-chip and on-chip memory. 
    However, the fusion dataflow for attention mechanisms on edge devices can be further optimized by using stream processing pipelines to enable semi-synchronous parallelization. This optimization is addressed by our proposed MAS-Attention in this paper.

